Classifying geospatial objects from multiview aerial imagery using semantic meshes

Aerial imagery is increasingly used in Earth science and natural resource management as a complement to labor-intensive ground-based surveys. Aerial systems can collect overlapping images that provide multiple views of each location from different perspectives. However, most prediction approaches (e.g. for tree species classification) use a single, synthesized top-down "orthomosaic" image as input that contains little to no information about the vertical aspects of objects and may include processing artifacts. We propose an alternate approach that generates predictions directly on the raw images and accurately maps these predictions into geospatial coordinates using semantic meshes. This method$\unicode{x2013}$released as a user-friendly open-source toolkit$\unicode{x2013}$enables analysts to use the highest quality data for predictions, capture information about the sides of objects, and leverage multiple viewpoints of each location for added robustness. We demonstrate the value of this approach on a new benchmark dataset of four forest sites in the western U.S. that consists of drone images, photogrammetry results, predicted tree locations, and species classification data derived from manual surveys. We show that our proposed multiview method improves classification accuracy from 53% to 75% relative to an orthomosaic baseline on a challenging cross-site tree species classification task.

==> figures/dataset.tex <==
\begin{figure*}[h]
  \centering
   \begin{subfigure}{0.33\linewidth}
   \centering
   \includegraphics[trim={2cm 4cm 1cm 4cm},clip, width=0.8\linewidth]{figures/imgs/dataset/geospatial_groundtruth.png}
   \caption{Geospatial groundtruth}
   \end{subfigure}
   \hfill
   \begin{subfigure}{0.33\linewidth}
   \centering
   \includegraphics[width=0.8\linewidth]{figures/imgs/dataset/photogrammetry.png}
   \caption{Photogrammetry}
   \end{subfigure}
   \hfill
   \begin{subfigure}{0.33\linewidth}
   \centering
   \includegraphics[width=0.8\linewidth]{figures/imgs/dataset/DTM.jpg}
   \caption{Digital terrain model}
   \end{subfigure}
  \caption{PLACEHOLDER: A figure showing the main components of the dataset.}
  
  \label{fig:dataset}
\end{figure*}

==> figures/labeled_mesh.tex <==
\begin{figure}
  \centering
  \includegraphics[trim={0 0 0 0 },clip,width=0.8\linewidth]{figures/imgs/labeled_mesh.png}
  \caption{A mesh labeled with species classes using geospatial ground truth data.}
  \label{fig:textured_mesh}
\end{figure}

==> figures/labeling_pipeline.tex <==
\begin{figure*}[h]
  \centering
   \begin{subfigure}{0.32\linewidth}
   \centering
   \includegraphics[width=\linewidth]{figures/imgs/labeling_pipeline/chips_fr.png}
  \label{fig:labeling_pipeline:gt_data}
   \caption{Geospatial ground truth data}
   \end{subfigure}
   \hfill
   \begin{subfigure}{0.64\linewidth}
   \centering
   \includegraphics[width=\linewidth]{figures/imgs/labeling_pipeline/chips_gt_mesh_no_ground_no_cams_cropped.png}
   \caption{Labeled mesh}
   \label{fig:labeling_pipeline:labeled_mesh}
   \end{subfigure}
  \caption{The classification labels from the geospatial ground truth data are applied to the mesh from the training site.}
  \label{fig:labeling_pipeline}
\end{figure*}

==> figures/qualitative_mesh.tex <==
\begin{figure*}
  \centering
   \begin{subfigure}{0.3\linewidth}
   \includegraphics[width=\linewidth]{figures/imgs/qualitative_mesh/colored_mesh.png}
   \caption{The mesh with the original RGB colors.}
   \end{subfigure}
   \begin{subfigure}{0.3\linewidth}
   \includegraphics[width=\linewidth]{figures/imgs/qualitative_mesh/pred_mesh.png}
   \caption{The mesh with the predicted classes}
   \end{subfigure}
   \begin{subfigure}{0.3\linewidth}
   \includegraphics[width=\linewidth]{figures/imgs/qualitative_mesh/gt_mesh.png}
   \caption{The mesh with the groundtruth classes}
   \end{subfigure}
  \caption{PLACEHOLDER: A figure showing the multiple versions of the same mesh}
  
  \label{fig:qualitative_mesh}
\end{figure*}

==> sec/2_ARCHIVED_background.tex <==
\section{Background}
\label{sec:background}
This work combines themes from several fields to perform machine learning for multiple views in three dimensions.
\subsection{Projective geometry}
Projective geometry is used in computer vision to model the relationship between a 3D scene and camera images of that scene. A camera is represented by two sets of parameters: intrinsic and extrinsic. Extrinsic parameters describe the camera's location and orientation with respect to the arbitrarily-defined world frame. Intrinsic parameters capture the relationship between points defined in the camera's coordinate system and pixels in the captured image. A detailed description of these concepts can be found in Multiple View Geometry by Hartley and Zisserman \cite{Hartley2004}.
\subsection{Meshes} Meshes are a data structure used in graphics computer vision that are commonly used to represent 3D objects as vertices and faces. Vertices are a collection of points in 3D space. Faces are a set of triangles connecting vertices. Faces are generally described by a three-tuple of integer indices into the set of vertices.
\subsection{Structure from motion}
\label{sec:background:SfM}
Structure from motion is a technique using a set of images to predict (a) camera lens parameters, (b) the pose (position and orientation) of the camera at each image capture, and (c) a 3D point cloud and/or mesh model of the scene using only a set of images (optionally aided by ballpark camera pose metadata). Early academic work was performed by \cite{Agarwal2009}, and more recently robust software such as Agisoft Metashape \cite{Agisoft2021}, COLMAP (ref), and OpenDroneMap (ref) has been developed for the task.
\subsection{Geospatial data} 
There are two common types of geospatial data: vector and raster. Vector data is represented by geometric objects such as points, lines, and closed polygons. In addition to these geometries, geospatial data possesses a coordinate reference system (CRS). A CRS defines how to interpret the coordinates of the geometry as locations on the earth surface. Furthermore, geometries (e.g., treetop points or tree crown polygons) can have associated attributes (e.g., height and species). Raster data is represented as top-down (orthographic) images of the world, with rows and columns of pixels represented by integers or floats. As with images, there can also be multiple channels of data (i.e., multiple values per pixel). Geospatial raster data possesses a transformation that can be used to determine the location of a given pixel on the earth.
As with vector data, raster data also has a CRS that describes how to interpret these coordinates as locations in the world. 
The resolution---or size of a pixel in spatial units---is known as the ground sample distance (GSD). 
\subsection{Orthomosaics}
\label{sec:background:orthomosaic}
An orthomosiac is a stitched top-down image of a photogrammetry scene. It is a type of geospatial raster data, usually containing the same number of bands as the input imagery. The details of how an orthomosaic is generated vary by software, but it generally uses the pose (position and orientation) of the camera at each image capture and the estimated 3D geometry of the scene, both of which are estimated using a structure from motion algorithm.
\subsection{Supervised machine learning}
Supervised machine learning involves training a model to generate predictions based on labeled examples. In many modern settings using images, these predictions are generated using deep learning. Deep learning leverages models containing a large number of parameters that are often trained with a variant of gradient descent. In this work, we refer to supervised machine learning simply as ML. 



==> sec/7_ARCHIVED_results.tex <==
\section{Results}
\label{sec:results}
\input{figures/quantitative_cf}
\input{tables/accuracy_table}
For each of the four sites, one set of predictions was generated using the orthomosaic and one using the multiview approach. In all cases, the site that was predicted was excluded from the training data. Site-level performance for both approaches is shown in \ref{table:per_site_accuracy}. 
In this analysis we compute the binary recall and binary precision per class, and macro-average these metrics across classes to highlight the performance on rarer classes (though the rarest class always represented > x \% of the observations). We also aggregate (sum) the confusion matrices across all sites and using these confusion matrices compute the accuracy, recall (macro-averaged by class) and precision (also macro-averaged by class). The aggregated confusion matrices can be found seen in Figure \ref{fig:quantitative_cf}. The Appendix contains the per-site confusions matrices in Figure \ref{fig:all_cf_matrices} and species-level analysis in Figure \ref{table:class_accuracy}.

In every instance of comparison, the multiview approach performed better than the orthomosaic approach. On the aggregate metrics, there was a major improvement from 52\% to 76\% on accuracy, 43\% to 69\% on recall, and 52\% to 75\% on precision. This demonstrates that the multiview approach is more accurate overall and also performs better on the rare classes. The performance on rare classes is further highlighted in Figure \ref{fig:quantitative_cf}. This shows that the orthomosaic approach dramatically over-predicts the two most common classes, PIPJ and PSME, while the distribution predicted by the multiview approach much more closely matches the real distribution.

%\subsection{Predictions on large unlabeled scenes}
%The goal of this work is to generate predictions on large regions. We did that for wow factor (and maybe so people can use this data cleverly in model training) but these predictions do not contribute to our analysis.
%\subsection{Compute and runtime considerations}
%One important factor to consider is the multi-view approach does require more computational resources. Here are some numbers describing that. However, model training dominates the computation in many situations. 

==> sec/Z_scratch-derek.tex <==
DEREK SCRATCH

omitting the often numerous oblique views present in the raw 2D imagery that could inform object detection and characterization. 

, provide a highly flexible and low-cost means for collecting high-resolution imagery (refs). 

 in part because the resulting imagery is generally of very high spatial resolution (e.g., 1-100 cm) {refs for NAIP, NEON AOP, Drone}.


The standard approach to mapping using drone imagery involves flying a series of contiguous transects to collect a grid of images with substantial (70-90\%) overlap with all neighbors. These images are usually then stitched and "orthorectified" onto a 3D surface of the scene estimated using a "structure from motion" algorithm (SEE SECTION 2). 




Classification of tree species using remote sensing data has been a highly active field of research for at least two decades (ref). An initial focus on multispectral satellite imagery has expanded in recent years to include species prediction from aerial imagery, generally driven by artificial neural network-based computer vision algorithms. For example, using transfer learning applied to RGB (red, green, blue) drone imagery, researchers have trained CNNs to identify Amazonian palms to species (among four options) based on orthoimagery with recall > 95\% (Ferreira et al. 2020), to distinguish between seven Japanese tree species classes using orthoimagery with F score > 0.85 (Onishi and Ise 2021), and to detect a specific tree species of concern among urban trees using raw drone images with F score > 0.90 (Santos et al. 2019). Approaches to species classification include (a) first cropping out individual (unclassified) tree crowns detected by other methods and then applying a classification algorithm (Onishi and Ise 2021), (b) applying pixel-level semantic segmentation to orthoimagery and then defining objects as clusters of pixels of the same class (Ferreira et al. 2020), or (c) applying architectures such as YOLO (REF) that simultaneously detect objects and classify them (Santos et al. 2019). Most often, species classes are obtained through manual, direct annotation of images by experts, which may inflate accuracy because human annotators observe the same images as the vision algorithm and may make similar errors (REF?). Using a more robust approach of assigning tree species classes through field-based surveys, Marconi et al. (2022) classified 72 species in a continental-scale survey using pixel-based non-computer vision  classification of hyperspectral imagery (426 reflectance bands) and a site identity predictor with F = 0.77, with spatially discrete observations from each site represented in both the training and testing samples. Weinstein at al. (2023) built on this approach to more accurately classify rare species at one site by developing a taxonomically hierarchical, multi-temporal computer vision-based modeling approach. Although some tree species classification work has leveraged imagery of the same objects from multiple time points and multiple sensors (Weinstein et al. 2023, Ahlswede et al. 2023)

==> tables/accuracy_table_old.tex <==
\begin{table*}[h!]
\begin{center}
\begin{tabular}{||c || c c | c c | c c | c c || cc ||} 
 \hline
 & \multicolumn{2}{c|}{Chips} & \multicolumn{2}{c|}{Delta} & \multicolumn{2}{c|}{Lassic} & \multicolumn{2}{c||}{Valley} & \multicolumn{2}{c||}{Aggregated}\\ [0.5ex] 
 & Ortho & MV & Ortho & MV & Ortho & MV & Ortho & MV & Ortho & MV  \\ [0.5ex] 
 \hline\hline
 Accuracy & 0.57 & 0.83 & 0.62 & 0.78 & 0.27 & 0.53 & 0.84 & 1.00 & 0.54 & 0.76 \\ \hline
 Recall & 0.51 & 0.64 & 0.47 & 0.69 & 0.52 & 0.74 & 0.81 & 1.00 & 0.46 & 0.70 \\ \hline
 Precision & 0.57 & 0.68 & 0.47 & 0.74 & 0.43 & 0.60 & 0.78 & 1.00 & 0.53 & 0.72 \\ \hline
\end{tabular}
\end{center}
\caption{Leave-one-out evaluation at the site level. Accuracy, macro-averaged recall, and macro-averaged precision are reported. The aggregated results across the sites are also reported, by summing the confusion matrices across all sites and then computing summary statistics. The multiview approach outperforms the orthomosaic method on every metric across all sites.}
\label{table:per_site_accuracy}
\end{table*}
